Tabletop Object Rearrangement: Structure, Complexity, and Efficient Combinatorial Search-Based Solutions

This thesis provides an in-depth structural analysis and efficient algorithmic solutions for tabletop object rearrangement with overhand grasps (TORO), a foundational task in advancing intelligent robotic manipulation. Rearranging multiple objects in a confined workspace presents two primary challenges: sequencing actions to minimize pick-and-place operations - an NP-hard problem in TORO - and determining temporary object placements ("buffer poses") within a cluttered environment, which is essential yet highly complex. For TORO with available external free space, this work investigates the minimum buffer space, or "running buffer size," required for temporary relocations, presenting both theoretical insights and exact algorithms. For TORO without external free space, the concept of lazy buffer verification is introduced, with its efficiency evaluated across various manipulator configurations, including single-arm, dual-arm, and mobile manipulators.

==> chapters/related.tex <==

\chapter{Related Works}
\thispagestyle{myheadings}

\section{Task and Motion Planning}
Human activities are generally driven by Task and Motion Planning (TAMP), which provides a natural model for robot planning. 
%
In recent years, integrated Task and Motion Planning (TAMP) \cite{garrett2021review} has been extensively studied, yielding significant advancements. 
%
\cite{toussaint2015logic} proposes logic-geometric programming, resulting in an optimization-based approach, to solve combined task and motion planning. \cite{dantam2016incremental,dantam2018incremental} tackles the challenges via incrementally incorporating additional planning constraints. \cite{kaelbling2011hierarchical} approaches integrated TAMP through a hierarchical planning framework. In that regard,  \cite{wang2022hierarchical} investigates how to generate hierarchical policies for grasping tasks in cluttered scenes with latent plans. 
%
Lately, \cite{luo2024Multistage} also utilizes hierarchical TAMP to resolve a multi-stage cable routing problem. \cite{wells2019learning} improves the scalability of TAMP in tabletop scenarios in the setup with one fixed robot by introducing geometric knowledge into the task planner. As task plan may require an ordered description, \cite{garrett2020pddlstream} defined PDDL (Planning Domain Definition Language) for task planning description, and \cite{zhao2023llm, chang2023lgmcts} utilizes LLM (large language model) to encode commonsense knowledge for task planning. \cite{kim2022representation} explores the representation, learning, and planning algorithms for geometric task and motion planning.

Despite recent advances, TAMP remains a major computational challenge due to its high computational complexity. 
Task planning works with discrete space and is frequently NP-hard \cite{han2018complexity,gaorunning}. Motion planning, on the other hand,  works with continuous space and is known to be PSPACE-hard \cite{hopcroft1984complexity}. 
Put together, finding feasible solutions to long-horizon TAMP is rather difficult; finding optimal solutions is generally out of the question. 





\section{Object Rearrangement}
Object rearrangement is a TAMP challenge with vast applications. NAMO (Navigation among Movable Obstacles) \cite{stilman2005navigation, stilman2008planning}, a class of well-studied problems in the domain, focuses on robot navigation through a space with many movable obstacles that the robot can manipulate. When NAMO instances satisfy certain properties, e.g., monotonicity or linearity, the plan search process can be simplified \cite{okada2004environment, stilman2005navigation, stilman2008planning, levihn2013hierarchical}. 
%
More recently, rearranging objects on tabletop and shelves  \cite{gao2021fast, cosgun2011push, wang2021uniform, gaorunning, wang2021efficient} have gained attention, in which a robot rearranges multiple objects to pre-defined goal poses. 
%
In object retrieval \cite{nam2019planning, ZhangLu-RSS-21, vieira2022persistent, huang2022self, huang2021dipn} objects must also be rearranged, but no pre-defined goals for all objects are given. 

Researches in robotics rearrangement consider various motion primitives. \cite{cosgun2011push, king2017unobservable, vieira2022persistent, huang2021dipn, huang2023optimal} use simple and low-cost but inaccurate non-prehensile actions such as push, some other works \cite{krontiris2015dealing, krontiris2016efficiently, wang2021efficient} use more accurate but higher-cost prehensile actions such as grasp.
Due to the inaccuracy of non-prehensile actions, it is hard to predict the resulting state after actions, which obstructs long-horizon planning.
Recent works\cite{king2017unobservable, huang2023optimal} maintain a Monte Carlo tree to decide the next action.
Since calling a physics simulator for rolling out is time-consuming, \cite{huang2021dipn} proposes a push prediction model to predict the state after a push.
With prehensile actions, the resulting states are more predictable.
Planners with prehensile actions \cite{bereg2006lifting, han2018complexity, nam2019planning, gaorunning} often emphasize the task planning challenges inherent in rearrangement tasks. Efficient and effective algorithms \cite{han2018complexity, gaorunning, bereg2006lifting} are developed through converting multi-object rearrangement problems to well-established graph-based discrete optimization problems. Collision-free workspace locations must be allocated for temporary object storage if external free space is unavailable \cite{krontiris2016efficiently,cheong2020relocate,gao2021fast,gao2023utility}. 
Besides rearrangement with a single robot arm, recent works also study scenarios with two fixed arms\cite{gao2022toward,gao2024toward} or a mobile manipulator\cite{gao2023orla}.


\section{Multi-Arm Rearrangement}
Multi-robot rearrangement requires additional computation on task assignment and coordination.
Ahn et al.\cite{ahn2021coordination} coordinate robots by maximizing the number of ``turn-taking'' moments when one arm is picking an obstacle from the workspace while the other arm is placing the previous obstacle at the external space.
Shome et al.\cite{shome2021fast} assume robot arms pick-n-places simultaneously and only solve monotone rearrangement problems, where each object can move directly to the goal pose.
For objects that need to be moved to a pose outside the reachable region of a robot arm,
the task can be accomplished by coordinating multiple arms to handoff the objects around\cite{shome2020synchronized}.
Cooperative pick-n-place, a problem related to multi-arm rearrangement, is well-studied in the area of printed circuit board assembly tasks\cite{li2008enhancing,moghaddam2016parallelism}. 
These problems do not have ordering constraints on pick-n-place tasks, i.e. all the items can move directly to goal poses in any ordering.
Research in these topics tends to consider multiple grippers equipped on a single arm rather than multiple arms, which reduces system flexibility.
Our previous work\cite{gao2022toward} studies dual-arm rearrangement in a shared workspace and coordinates two arms for task sequencing of pick-n-place and handoff primitive actions.

In terms of motion planning, typical manipulators (robot arms) have six degrees of freedom. Planning motion for a $k$-arm system must navigate a very high $6k$-dimensional space.
%
Computationally, High-dimensional path/motion planning is exceptionally challenging. Typical planners for this purpose fall into two categories: Sampling-based \cite{karaman2011sampling, janson2018deterministic, Ichter2018Learning, gammell2014informed, RRT, PRM} and optimization-based \cite{schulman2014motion, zucker2013chomp, marcucci2023motion, urain2023se, malyuta2022convex}. 
A prevailing approach for high-dimensional motion planning is sampling-based rooted in, e.g., PRM \cite{PRM} and RRT \cite{RRT}, with subsequent and ongoing improvements including RRT*\cite{karaman2011sampling}, SST \cite{li2016asymptotically}, AO-RRT \cite{hauser2016asymptotically}. Recently, VAMP \cite{thomason2023motions} has shown promising results by utilizing AVX2-based parallelization to accelerate forward kinematics and collision-checking computation. 
%
An optimization-based approach generates trajectories with incremental optimizations based on specific constraints and cost functions. Representative algorithms include CHOMP \cite{zucker2013chomp} and TrajOpt \cite{schulman2014motion}. More recently, \cite{marcucci2023motion} developed convex optimization-based motion planning around obstacles.  \cite{zhang2023provably} implements a Semi-Infinite Program solver to provide provably robust collision avoidance. \cite{urain2023se} studies using diffusion to design smooth joint cost functions for grasp and motion planning. \cite{malyuta2022convex} investigates generating feasible trajectories considering dynamics.
%
cuRobo \cite{curobo} leverages GPU to speed up graph search for trajectory planning and optimization, significantly improving planning time and trajectory quality.
Our recent work\cite{gao2024toward} uses cuRobo for efficient planning in the 12 DoF dual-arm configuration space.

\section{Buffer Pose Allocation in Rearrangement Planning}
In the realm of rearrangement problems, there are instances where specific objects cannot be moved directly to their intended goal poses. 
These scenarios compel the temporary movement of objects to collision-free poses. 
To streamline the rearrangement planning, several rearrangement methodologies exploit external free spaces as buffer zones\cite{gao2023minimizing,xu2023optimal}. 
One notable concept is the \emph{running buffer size}\cite{gao2023minimizing}, which quantifies the requisite size of this external buffer zone. 
In situations devoid of external space for relocation, past research either pre-identifies potential buffer candidates\cite{wang2021uniform,cheong2020relocate} or segments the rearrangement tasks into sequential subproblems\cite{krontiris2016efficiently,wang2022lazy}.
TRLB\cite{gao2022fast}, aiming for an optimized buffer selection, prioritizes task sequencing and subsequently employs the task plan to dictate buffer allocation. 
However, TRLB doesn't factor in travel costs. 
Contrarily, in our latest study\cite{gao2023orla}, we incorporate lazy buffer allocation within the \astar search and prioritize buffer poses based on various cost function optimizations.
Besides that, the study introduces a deep-learning-based prediction model, \model, to estimate the stability of buffer poses on top of other objects.
